Cascade Pipeline for Leading-Order Matrix Element Evaluation on AMD Versal AI Engine Arrays

A major computational bottleneck in modern High Energy Physics event generators arises from the integration of the matrix element, which requires repeated evaluations at different phase-space points to cover all possible initial- and final-state configurations. As the Large Hadron Collider enters its High-Luminosity phase, the demand for energy-efficient acceleration is expected to exceed the limits of conventional CPU scaling, motivating the use of highly parallel computing platforms such as graphics processing units (GPUs). In this work, we present an alternative approach based on a cascade pipeline architecture for evaluating leading-order matrix elements of the \ggttg process on AMD Versal AI Engine (\aie) arrays. Due to the 16\,kB per-tile program memory constraint, the computation is decomposed into a five-stage pipeline, with stages communicating via a wavefunction-token protocol over the on-chip cascade interface. Mapping 80 independent pipelines onto the 400 \aie tiles of the VCK190 platform yields a projected throughput of $1.0\times10^6$ matrix element evaluations per second at 54.8\,W, corresponding to a $34\times$ speedup over a single CPU core and a $7.7\times$ improvement in energy efficiency. Numerical agreement with the \amcnlo double-precision reference is validated at the parts-per-million level in mean relative error.

==> sec_platform.tex <==
%% sec_platform.tex
%% ─────────────────────────────────────────────────────────────────────────────
%% Section 3 — Target Platform: AMD Versal AI Engine Architecture
%% ─────────────────────────────────────────────────────────────────────────────

\section{Target Platform: AMD Versal AI Engine Architecture}\label{sec:platform}

\subsection{Device overview}

The AMD Versal AI Core Series VCK190 evaluation kit is built around the
XCVC1902 Adaptive Compute Acceleration Platform (ACAP).  The device integrates
three compute domains on a single die: a dual-core ARM Cortex-A72 application
processor (1.7\,GHz) used for system control and host orchestration; a
dual-core ARM Cortex-R5F real-time processor; and the programmable logic (PL)
fabric with 899\,840 LUTs, 1\,968 DSP58 engines, and 158\,MB of embedded
memory (UltraRAM + BRAM).  The AI Engine array is the key resource for
computation in this work.

\subsection{AI Engine tile microarchitecture}\label{sec:aie_tile}

The device contains \textbf{400 \aie tiles} arranged in a $50\times 8$ array
and clocked at 1\,GHz.  Each tile comprises:
\begin{itemize}
  \item A 512-bit SIMD vector unit supporting single-precision (float32) and
    fixed-point arithmetic;
  \item A 32-bit scalar RISC core for control flow;
  \item 32\,kB of local data memory (plus 128\,kB addressable via neighbours);
  \item \textbf{16\,kB of dedicated program memory (PM)}---the hard constraint
    that drives the architecture of this work.
\end{itemize}

\subsection{Cascade interface}\label{sec:cascade}

Adjacent tiles in the same row are connected by a \textbf{cascade interface}:
a 384-bit unidirectional accumulator bus clocked in lock-step with the vector
pipeline.  Key properties relevant to this work are:
\begin{itemize}
  \item \textbf{Deterministic, zero-overhead data transfer}: one 384-bit word
    ($4\times\texttt{cfloat}$) per clock cycle, no flow-control signals.
  \item \textbf{Hardware FIFO}: a 4-entry FIFO decouples producer and consumer
    by up to 4 cycles, absorbing minor skew without stalling.
  \item \textbf{Fixed direction per row}: even rows (0, 2, 4, 6) cascade
    left-to-right; odd rows (1, 3, 5, 7) cascade right-to-left.  Kernel
    placement must match this hardware topology.
  \item \textbf{Bandwidth}: $384\,\text{bits}/\text{cycle} \times 1\,\text{GHz}
    = 48\,\text{GB/s}$, far exceeding the stream I/O bandwidth from the shim.
\end{itemize}

\subsection{Stream switching and PLIO}

Tiles communicate with the PL through \emph{Programmable Logic I/O} (PLIO)
ports at the shim row.  On XCVC1902, valid shim columns for PLIO placement are
columns 6--43 (columns 0--5 and above 43 host AIE-PL interface tiles but not
direct PLIO sites).  The stream switch network routes packets between tiles
using packet headers, enabling \texttt{pktsplit} and \texttt{pktmerge}
primitives that distribute or collect one stream to/from multiple tiles without
dedicated PL logic.

\subsection{Program memory as the primary constraint}

Unlike GPU or CPU codebases where code size is virtually unconstrained, the
16\KB PM limit is hard and non-negotiable.  A kernel that overflows PM cannot
be compiled.  Table~\ref{tab:pm_footprint} quantifies the PM contribution of
each HELAS function used in \ggttg, establishing why no single tile can hold
the complete computation.

\begin{table}[h]
\caption{Estimated program memory footprint of each HELAS function used for
\ggttg on the \aie.  Values are representative; exact figures depend on
compiler optimisation flags.  The 16\KB hardware limit is shown for
reference.}
\label{tab:pm_footprint}
\begin{tabular}{@{}lrl@{}}
\toprule
HELAS function / component & PM (bytes) & Used in \\
\midrule
\texttt{VVV1P0\_1} (off-shell gluon)          & ${\sim}2{,}000$ & K1 \\
\texttt{FFV1P0\_3} (off-shell boson)          & ${\sim}2{,}700$ & K3 (moved) \\
\texttt{FFV1\_0/1/2} (FFV amplitudes)         & ${\sim}4{,}400$ & K2a, K2b \\
\texttt{VVV1\_0} (triple-gluon amplitude)     & ${\sim}2{,}100$ & K3 \\
\texttt{VVVV1/3/4P0\_1} (4-gluon contact)    & ${\sim}6{,}600$ & K4 \\
Kernel logic + token serialisation            & ${\sim}11{,}000$ & all \\
Softfloat runtime                             & ${\sim}1{,}500$ & all \\
\midrule
\textbf{Monolithic total}                     & ${\sim}38{,}000$ & --- \\
\textbf{16\KB hardware limit}                 & $16{,}384$ & --- \\
\bottomrule
\end{tabular}
\end{table}

The \textbf{VVV Exclusion Principle} emerges directly from
Table~\ref{tab:pm_footprint}: \texttt{VVV1P0\_1} (${\sim}2.0\KB$) and
\texttt{VVV1\_0} (${\sim}2.1\KB$), when combined with the kernel logic
overhead, cannot coexist in a single 16\KB tile.  They must reside in
separate kernels---\texttt{K1} and \texttt{K3} respectively.

